Zero-Shot Sketch Based Image Retrieval using Graph Transformer

The performance of a zero-shot sketch-based image retrieval (ZS-SBIR) task is primarily affected by two challenges. The substantial domain gap between image and sketch features needs to be bridged, while at the same time the side information has to be chosen tactfully. Existing literature has shown that varying the semantic side information greatly affects the performance of ZS-SBIR. To this end, we propose a novel graph transformer based zero-shot sketch-based image retrieval (GTZSR) framework for solving ZS-SBIR tasks which uses a novel graph transformer to preserve the topology of the classes in the semantic space and propagates the context-graph of the classes within the embedding features of the visual space. To bridge the domain gap between the visual features, we propose minimizing the Wasserstein distance between images and sketches in a learned domain-shared space. We also propose a novel compatibility loss that further aligns the two visual domains by bridging the domain gap of one class with respect to the domain gap of all other classes in the training set. Experimental results obtained on the extended Sketchy, TU-Berlin, and QuickDraw datasets exhibit sharp improvements over the existing state-of-the-art methods in both ZS-SBIR and generalized ZS-SBIR.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> rebuttal.tex <==
% \documentclass{article}

% \usepackage[a4paper, total={6.5in, 9.5in}]{geometry}
% \usepackage[utf8]{inputenc}
% \usepackage{lipsum}
% \usepackage{framed}
% \usepackage{color}
% \usepackage{amsfonts}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage[pdftex]{graphicx}     
% \usepackage{capt-of}
% \usepackage{graphics}
% \usepackage{graphicx}
% \usepackage{multicol}
% \usepackage{multirow}
% \usepackage{colortbl} %newwwwwwww
% \usepackage{url}
% \usepackage{hyperref}
% \usepackage{siunitx} 
% \usepackage[caption=false]{subfig}

% \usepackage{pifont}% http://ctan.org/pkg/pifont
% \newcommand{\ushasi}[1]{\textcolor{red}{Ushasi: #1}}


% \usepackage{graphbox} %loads graphicx package
% \usepackage{booktabs}
% \usepackage{mathtools}

% \usepackage[ruled,vlined]{algorithm2e}
% \usepackage{algorithmicx}
% \usepackage{flushend}
% \usepackage{algpseudocode}

% \definecolor{mygray}{gray}{0.3}
% \setlength{\parskip}{1em}
% \newcommand{\etal}{\textit{et al}.}

% \newenvironment{reply} 
% {\begin{leftbar} \noindent \textsc{\textbf{} } \newline \color{blue}} 
% {\end{leftbar}}{ \vspace{5mm}}

% \setlength{\parindent}{0pt}
% \newenvironment{point}[1][0]{ \noindent \textbf{\textsc{(Point #1)}} \color{mygray}  \itshape  }{ \vspace{5mm}}

% \newenvironment{reviewer}[1][0]{ \noindent \vspace{6mm} \\ \textsc{\textbf{\huge Reviewer #1}} \color{black} \vspace{3mm} \\ }{\vspace{5mm}\hrule \vspace{5mm} }

% \title{Reply to Reviewers Comments : ICPR 2022 - 1332} 

% \begin{document}

% \begin{center}{Response to Reviewers' Comments on ICPR 2022 - 1332 \\
% \vspace{5mm}
% \Large \textbf{Zero-Shot Sketch Based Image Retrieval using Graph Transformer}} 
% \end{center}

% This manuscript was submitted to ICPR 2022 (1332). As per the reviewers' suggestions, it is now revised and submitted to the same along with the responses to comments from the reviewers. The authors are indebted to the anonymous reviewers for their constructive criticism, which has been instrumental in improving the technical quality of the manuscript. {The authors are most appreciative to the Editors and the Associate Editor for performing the prompt review process and highlighting critical viewpoints to enhance the quality of the manuscript.}

% In the following we transcribe the comments in \textcolor{mygray}{\emph{gray italics}}, and our responses in \textcolor{blue}{blue} in a \textbf{response} section. The changes are highlighted in \textcolor{red}{red} in the revised manuscript. 



% \begin{reviewer}[1]
% \textbf{Reviewer 12475:} In this paper, the authors propose a novel graph
% transformer based zero-shot sketch-based image retrieval
% (GTZSR) framework for solving ZS-SBIR tasks. They uses a
% graph transformer to preserve the topology of the classes
% in the semantic space and propagates the context-graph of
% the classes within the embedding features of the visual
% space. Experimental results the proposed solution exhibit
% sharp improvements over the existing state-of the-art
% methods in both ZS-SBIR and generalized ZS-SBIR. Their work
% is interesting and innovative. The authors also undertake
% sufficient comparative experiments.


% \begin{reply}
% The authors are very appreciative to the reviewer for recognizing and appreciating our work.  

% \end{reply}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \end{reviewer}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %\newpage
% \begin{reviewer}[2]
% \textcolor{mygray}{\textbf{Reviewer 16029:} The paper is very well-written and the motivation of the
% task is well-defined in the introduction, along with a
% section of ‘problem formulation’ in the methodology for
% proper understanding. The authors talk about the utility of
% semantic spaces and say the topology of the semantic space
% is key to solving the problem of ZS-SBIR. The utility of
% GCN in this scenario is discussed. 3 contributions have
% been claimed: 1)2 alignment losses between sketch and image
% modalities 2)A new GTN layer introduced in the semantic
% space on top of GCN to preserve contextual graph
% information 3) Substantial gain in benchmark evaluation
% metrics on both Z-SBIR and (G)-Z-SBIR tasks.}
% \begin{reply}
% The authors are very appreciative to the reviewer for recognizing and appreciating our work.  

% \end{reply}
% %%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{point}[1]
% The highlight of this work relies on the usage of GTN that use multi-hop connection to learn improved node representations in the semantic space. In Table 2  ablation, they justify the power of GTNs showing a 22 percent fall in performance w/o its usage. Although the architecture in terms of novelty is limited (except introducing the GTN layer on top of GCN), the study of the learning objectives introduced in the pipeline is interesting.  In paragraph 3 line 4 of Section 1, there’s a type error “P@100values”... the method overall adopts a similar structure to the Doodle2Sketch (Dey et. al.) pipeline with the introduction of GTN and GCN modules in
% the semantic space. Also, the triplet-loss based network is substituted by a compatibility loss(like an Info-NCE) and a domain alignment loss(variational loss on minimizing Wasserstein distance). 
% \end{point}
% %
% \begin{reply}
% We are very thankful to the reviewers for their valuable oversights. The authors sincerely apologize for the grammatical and typing mistakes. They have been corrected in the revised manuscript.

% In this paper, we solve a ZS-SBIR problem and extend it for a GZS-SBIR setup. Our primary contribution is to propose a novel compatibility loss measure to bridge the domain gap between the two visual modalities of image and sketches. We also introduce a novel graph transformer network in conjunction with a graph convolution layer to preserve the context graph of the semantic space and exploit this knowledge it align the visual space. To help further align the image and sketch modalities, we propose minimizing the Wassterstein distance between the visual modalities so as to transform the distribution of images to sketches. To validate the efficacy of the proposed network, we perform extensive experiments on the standard benchmarked datasets of the extended Sketchy, TU-Berlin, and QuickDraw and outperform the existing state-of-the-art on all the evaluation metrices by $10-20\%$.

% A major research gap in the existing models that solves for ZS-SBIR tasks is that there is no common evaluative measure for all the papers. Some papers report their performances on precision@100 values, while some on precision@200 values, whichever gives better set of results. This makes the results incomparable with each other. In order to remove the inconsistencies, we prefer to put a complete set of results that should help in better comparison with all the state-of-the-art models. 


% \end{reply}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{point}[2]
% The discussions on the ablations prove to be the main insight of the approach, with very good performance gains in the existing benchmarks. I would encourage the authors to also try more optimal transport techniques (like the earth-mover distance/sinkhorn loss).
% \end{point}
% %
% \begin{reply}
% The authors are thankful to the reviewer for this suggestion. We tried using the Sinkhorn metric for minimizing the domain gap between the sketches and images and found the network's performance to be much lower than the Wasserstein metric in this ZS-SBIR problem. This could be possibly attributed to the fact that the Sinkhorn divergence blurs the transport plan through the addition of an entropic penalty. This helps in reducing the effective dimensionality of the transportation problem and compute sensible approximations of the Wasserstein distance at a low computational cost. Hence, in the trade-off between accuracy and efficiency, Wasserstein yields superior results.  

% In statistics, the earth mover's distance (EMD) is a measure of the distance between two probability distributions over a region. In mathematics, this is also known as the Wasserstein metric. 
% \end{reply}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{point}[3]
% Taking into consideration the substantial gain in benchmark performance and also good explanation and insights on the justification of the proposed pipeline, I would give an acceptance. I would also highly recommend the authors to publish a working open-source version of their work on github repo and more information on the implementation details (the values of lambdas in the overall loss function is missing), for the benefit of the SBIR research community for reproducibility given also. It would be nice if you could also include a supplementary if you cannot include all the details of implementation in the main paper.
% \end{point}
% %
% \begin{reply}
% The authors are very appreciative to the reviewer for recognizing and appreciating our work. 

% We are very thankful to the reviewers for their valuable oversights. We have published the codes online at GitHub at the following repository: \href{https://github.com/awesumrit/GTZSR}{https://github.com/awesumrit/GTZSR} for the benefit of the SBIR research community for reproducibility. We have also added more of the implementation details in the main manuscript.


% \end{reply}

% \end{reviewer}

% \end{document}
% \hrule


